Fast Multivariate Log-Concave Density Estimation

A novel computational approach to log-concave density estimation is proposed. Previous approaches utilize the piecewise-affine parametrization of the density induced by the given sample set. The number of parameters as well as non-smooth subgradient-based convex optimization for determining the maximum likelihood density estimate cause long runtimes for dimensions $d \geq 2$ and large sample sets. The presented approach is based on mildly non-convex smooth approximations of the objective function and \textit{sparse}, adaptive piecewise-affine density parametrization. Established memory-efficient numerical optimization techniques enable to process larger data sets for dimensions $d \geq 2$. While there is no guarantee that the algorithm returns the maximum likelihood estimate for every problem instance, we provide comprehensive numerical evidence that it does yield near-optimal results after significantly shorter runtimes. For example, 10000 samples in $\mathbb{R}^2$ are processed in two seconds, rather than in $\approx 14$ hours required by the previous approach to terminate. For higher dimensions, density estimation becomes tractable as well: Processing $10000$ samples in $\mathbb{R}^6$ requires 35 minutes. The software is publicly available as CRAN R package fmlogcondens.

==> related-work.tex <==
\section{Related Work}
This section mainly addresses the state-of-the-art approach by \cite{cule2010} for multivariate log-concave density estimation, who solve \eqref{eq:MLE-Silverman} for $d \geq 2$. An important ingredient of their approach is the following explicit form for the integral term, given a triangulation $\mc{T}_n$ of $\conv(X)$:
\begin{lemma}
Let $j = (j_0, \ldots, j_d)$ be a (d+1)-tupel of distinct indices in $\{1, \ldots, n\}$, such that $C_{n,i} = \conv(x_{j_0}, \ldots, x_{j_d})$ is a simplex with associated affine function $\vphi_{i,n} = \la a_i, x \ra + b_i$ and values $y_{j_l} = \vphi_{i,n}(x_{j_l})$ at its vertices. Then the integral $\int_{C_{n,i}} \exp(-\hat{\vphi}_{i,n}(x)) \dd{x}$ can be calculated as
\begin{equation}
\label{eq:exact-integral}
\int_{C_{n,i}} \exp(-\vphi_{i,n}(x)) \dd{x} = \mathrm{vol}(C_{n,i}) \sum_{l=0}^d \exp(-y_{j_l}) \prod_{i \in \{0, \ldots, d \} \setminus{\{l\}}} (y_{j_i} - y_{j_l})^{-1}. 
\end{equation}
\label{lemma:integral-cule}
\end{lemma}
A derivation can be found in \cite[Appx.~B.1]{cule2010}. The Lemma allows the explicit evaluation of the integral term in \eqref{eq:MLE-Silverman}, given a triangulation $\mc{T}_n$ such that each cell corresponds to a single linear function. Their final optimization problem is
\begin{equation}
L(y) =  -\frac{1}{n}\sum_{i=1}^n y_i + \sum_{\sigma \in \mc{T}_n} \mathrm{vol}(\sigma) \sum_{l=0}^d \frac{\exp(y_{j_l})}{\prod_{l\in \{0, \ldots, d \} \setminus{\{i\}}} (y_{j_i} - y_{j_l})^{-1}}.
\label{eq:MLE-Cule}
\end{equation}
While in general it holds that $L(h) \geq L(y)$ since $h_{X,y}(X_i) \geq y_i$, in the optimum we have $h_{X,y}(X_i) = y_i$ for all $i=1, \ldots, n$, since non-touching $y_i$'s can always be set to $h_{X,y}(X_i)$, thereby increasing $L(y)$ without altering the value of the integral term. Therefore both formulations \eqref{eq:MLE-Silverman} and \eqref{eq:MLE-Cule} yield the same optimal solution \citep{cule2010}. We will now point out limitations of this approach, that will motivate our alternative formulation introduced Section \ref{sec:method}.

The formulation \eqref{eq:MLE-Cule} is a \textit{non-smooth, convex} optimization problem. While convexity guarantees convergence to the global optimum, non-smoothness prevents the use of classical Newton's method or related approaches. Instead the authors rely on a subgradient method, which has at most linear convergence rate. Consequently, they observe a linear dependence between the number of iterations and $n$. 

A more severe limitation is the requirement to find the polyhedral subdivision $\mc{S}_n$ induced by the lifted point configuration $X^y$ and its \textit{refinement into a triangulation} $\mc{T}_n$ \textit{at each step of the optimization}, in order to evaluate \eqref{eq:MLE-Cule} and its gradient. While methodically this can be easily achieved using a convex hull solver such as \texttt{qhull} \citep{barber1996quickhull}, the worst-case complexity of this operation is $O(n\log n + n^{\lfloor d/2 \rfloor})$. The worst-case is approached close to the optimum $y^{*}$, since most $y_i$'s will lie on the surface of $h_{X,y}$ and thereby contribute to the convex hull of $X^y$.

%\begin{figure}
%\centering 
%\subfloat[][$n$-gon with $n=25$]{\includegraphics[width=0.32\textwidth]{fig/ngon}}
%\hfill
%\subfloat[][\centering \footnotesize{\cite{cule2010}, \par $L(y) = -29.4109$, $m=23$}]{\includegraphics[width=0.32\textwidth]{fig/ngon-cule}}
%\hfill
%\subfloat[][\centering \footnotesize{Our estimate, \par $L(\theta) = -29.4109$, $m=1$}]{\includegraphics[width=0.32\textwidth]{fig/ngon-ours}}
%\caption{(a) 25 data points that form a $n$-gon. Due to the symmetry of $X$, $\hat{f}_n$ for this example is the uniform density (not explicitly shown here, both approaches yield that estimate). What is crucial is the fact that this density can be represented by \textit{one} hyperplane corresponding to a polytope consisting all of $\conv(X)$. Our approach correctly finds that representation (c). In contrast the approach of Cule et al.~(b) relies on a triangulation of $\conv(X)$, which constitutes an overly complex representation of $h_{X,y}(x)$, since each simplex corresponds to a hyperplane with the same set of parameters.}
%\label{fig:n-gon}
%\end{figure}

Relying on a triangulation may constitute a \textit{massive overparametrization}, since it hides all potential maximal polytopes on which $h_{X,y}(x)$ is linear. As an illustrative example, consider a regular $n$-gon in $\R^2$, displayed for $n=25$ in Figure~\ref{fig:n-gon} (a). This example was suggested by Dominic Schuhmacher (University of Bern) in the discussion on the paper by \citet{cule2010}, to illustrate the shortcomings of the enforced triangulation. Due to the symmetry of the point set $X$, $\hat{f}_n$ is the uniform density, which can be expressed by a \textit{single} hyperplane. Thus the complexity of the underlying density for any $n$-gon is $O(1)$. On the other hand, triangulating a $n$-gon creates $n-2$ simplices, each with its own set of hyperplane parameters. Thus the solution of Cule et al.~(Figure~\ref{fig:n-gon} (b)) has $O(n)$ parameters in total.

As we demonstrate in Section~\ref{sec:results} of this paper, many examples exhibit such sparse representations which are hidden by the simplical decomposition $\mc{T}_n$. In order to be able to profit the aforementioned sparsity of the underlying density, we propose an alternative formulation for \eqref{eq:MLE-Silverman}, based on the dual representation for $h$ in terms of a set of hyperplane parameters $\theta$ \eqref{eq:polyhedral-convex-function}. Figure~\ref{fig:n-gon}~(c) demonstrates that our approach successfully found the `decomposition` of $\conv(X)$ into one maximal polytope. This work continues preliminary ideas examined in \cite{rathke2015b} for $\R^2$.

\subsection{Log-Concave Densities in $\pmb{\mathbb{R}}$}
The problem structure in $d=1$ is much simpler: There exist only one triangulation of $\conv(X)$ in $\R$. Furthermore, instead of defining the concave function $h(x)$ as a combinatorial optimization problem as in \eqref{eq:finitely-generated}, concavity of $h(x)$ can be expressed by a set of linear constraints on the slopes of neighboring affine functions. The resulting optimization problem is convex, smooth and can be solved using Newton-based methods, see for example \cite{rufibach2006thesis} and \cite{walther2002}. A much more efficient active set based approach was presented by \cite{rufibach2007}, which finds the optimum using the \textit{minimal} set of hyperplanes. In that sense it is similar to our approach, which tries to find a minimal representation of $f(x)$ in $\R^d$. We will compare our results to their approach for examples in $d=1$.

\subsection{Global Consistency and Rate of Convergence}
A lot of research was directed towards the theoretical properties of multivariate log-concave density estimation. \cite{Diakonikolas:2017aa} investigated lower and upper bounds on sample complexity in order to learn a log-concave density with total variation distance of at most $\epsilon$. We will compare their bounds to our empirical results. \todo{more...}
